Baxter $d$-permutations and other pattern avoiding classes

A permutation of size $n$ can be identified to its diagram in which there is exactly one point per row and column in the grid $[n]^2$. In this paper we consider multidimensional permutations (or $d$-permutations), which are identified to their diagrams on the grid $[n]^d$ in which there is exactly one point per hyperplane $x_i=j$ for $i\in[d]$ and $j\in[n]$. We first investigate exhaustively all small pattern avoiding classes. We provide some bijection to enumerate some of these classes and we propose some conjectures for others. We then give a generalization of well-studied Baxter permutations into this multidimensional setting. In addition, we provide a vincular pattern avoidance characterization of Baxter $d$-permutations.

==> patterns_2_1.tex <==
\perm{12}{12} & 4 & 1, 3, 17, 151, 1899, 31711, 672697, \ensuremath{\cdots} & \href{http://oeis.org/A007767}{A007767}? \\
\hline


==> patterns_2_1_2_1_mix.tex <==
12, \perm{12}{12} & 1 & 1, 0, 0, 0, 0, 0, 0, \ensuremath{\cdots} &  \\
\hline
12, \perm{12}{21} & 3 & 1, 0, 0, 0, 0, 0, 0, \ensuremath{\cdots} &  \\
\hline
21, \perm{12}{12} & 1 & 1, 0, 0, 0, 0, 0, 0, \ensuremath{\cdots} &  \\
\hline
21, \perm{12}{21} & 3 & 1, 1, 1, 1, 1, 1, 1, \ensuremath{\cdots} & 21 \\
\hline


==> patterns_2_1_3_1.tex <==
\perm{12}{12}, \perm{123}{123} & 4 & 1, 3, 17, 151, 1899, 31711, 672697, \ensuremath{\cdots} & \perm{12}{12}, \perm{123}{231}? \\
\hline
\perm{12}{12}, \perm{123}{132} & 24 & 1, 3, 17, 151, 1899, 31711, 672697, \ensuremath{\cdots} & \perm{12}{12}, \perm{123}{231}? \\
\hline
\perm{12}{12}, \perm{123}{231} & 24 & 1, 3, 17, 151, 1899, 31711, 672697, \ensuremath{\cdots} & \href{http://oeis.org/A007767}{A007767}? \\
\hline
\perm{12}{12}, \perm{123}{321} & 12 & 1, 3, 16, 124, 1262, 15898, 238572, \ensuremath{\cdots} & \href{http://oeis.org/A190291}{A190291}? \\
\hline
\perm{12}{12}, \perm{132}{213} & 24 & 1, 3, 17, 151, 1899, 31711, 672697, \ensuremath{\cdots} & \perm{12}{12}, \perm{123}{231}? \\
\hline
\perm{12}{12}, \perm{132}{312} & 48 & 1, 3, 16, 125, 1296, 16807, 262144, \ensuremath{\cdots} & \href{http://oeis.org/A000272}{A000272}? \\
\hline
\perm{12}{12}, \perm{231}{312} & 8 & 1, 3, 16, 122, 1188, 13844, 185448, \ensuremath{\cdots} & \href{http://oeis.org/A295928}{A295928}? \\
\hline


==> patterns_2_1_d2.tex <==
12 & 1 & 1, 0, 0, 0, 0, 0, 0, \ensuremath{\cdots} &  \\
\hline
21 & 1 & 1, 1, 1, 1, 1, 1, 1, \ensuremath{\cdots} & \href{http://oeis.org/A000012}{A000012}? \\
\hline


==> patterns_2_2.tex <==
\perm{12}{12}, \perm{12}{21} & 6 & 1, 2, 6, 24, 120, 720, 5040, \ensuremath{\cdots} & \href{http://oeis.org/A000142}{A000142}? \\
\hline


==> patterns_2_3.tex <==
\perm{12}{12}, \perm{12}{21}, \perm{21}{12} & 4 & 1, 1, 1, 1, 1, 1, \ensuremath{\cdots} & \href{http://oeis.org/A000012}{A000012}? \\
\hline


==> patterns_2d_2_1.tex <==
12 & 2 & 1, 1, 1, 1, 1, 1, 1, \ensuremath{\cdots} & \href{http://oeis.org/A000012}{A000012}? \\
\hline


==> patterns_2d_2_2.tex <==
12, 21 & 1 & 1, 0, 0, 0, 0, 0, 0, \ensuremath{\cdots} &  \\
\hline


==> patterns_2d_3_1.tex <==
123 & 2 & 1, 2, 5, 14, 42, 132, 429, \ensuremath{\cdots} & \href{http://oeis.org/A000108}{A000108}? \\
\hline
132 & 4 & 1, 2, 5, 14, 42, 132, 429, \ensuremath{\cdots} & 123? \\
\hline


==> patterns_2d_3_2.tex <==
123, 132 & 4 & 1, 2, 4, 8, 16, 32, 64, \ensuremath{\cdots} & \href{http://oeis.org/A000079}{A000079}? \\
\hline
123, 231 & 4 & 1, 2, 4, 7, 11, 16, 22, \ensuremath{\cdots} & \href{http://oeis.org/A000124}{A000124}? \\
\hline
123, 321 & 1 & 1, 2, 4, 4, 0, 0, 0, \ensuremath{\cdots} &  \\
\hline
132, 213 & 2 & 1, 2, 4, 8, 16, 32, 64, \ensuremath{\cdots} & 123, 132? \\
\hline
132, 231 & 4 & 1, 2, 4, 8, 16, 32, 64, \ensuremath{\cdots} & 123, 132? \\
\hline


==> patterns_2d_3_3.tex <==
123, 132, 213 & 2 & 1, 2, 3, 5, 8, 13, 21, \ensuremath{\cdots} & \href{http://oeis.org/A000045}{A000045}? \\
\hline
123, 132, 231 & 8 & 1, 2, 3, 4, 5, 6, 7, \ensuremath{\cdots} & 123, 231, 312? \\
\hline
123, 132, 321 & 4 & 1, 2, 3, 1, 0, 0, 0, \ensuremath{\cdots} &  \\
\hline
123, 231, 312 & 2 & 1, 2, 3, 4, 5, 6, 7, \ensuremath{\cdots} & \href{http://oeis.org/A000027}{A000027}? \\
\hline
132, 213, 231 & 4 & 1, 2, 3, 4, 5, 6, 7, \ensuremath{\cdots} & 123, 231, 312? \\
\hline


==> patterns_2d_3_4.tex <==
123, 132, 213, 231 & 4 & 1, 2, 2, 2, 2, 2, 2, \ensuremath{\cdots} & \href{http://oeis.org/A055642}{A055642}? \\
\hline
123, 132, 213, 321 & 2 & 1, 2, 2, 1, 0, 0, 0, \ensuremath{\cdots} &  \\
\hline
123, 132, 231, 312 & 4 & 1, 2, 2, 2, 2, 2, 2, \ensuremath{\cdots} & 123, 132, 213, 231? \\
\hline
123, 132, 231, 321 & 4 & 1, 2, 2, 0, 0, 0, 0, \ensuremath{\cdots} &  \\
\hline
132, 213, 231, 312 & 1 & 1, 2, 2, 2, 2, 2, 2, \ensuremath{\cdots} & 123, 132, 213, 231? \\
\hline


==> patterns_sym_3_1.tex <==
\Sym(\perm{123}{123}) & 4 & 1, 4, 32, 368, 4952, 68256, \ensuremath{\cdots} & \ensuremath{new} \\
\hline
\Sym(\perm{123}{132}) & 24 & 1, 4, 12, 4, 4, 4, \ensuremath{\cdots} & \ensuremath{new} \\
\hline
\Sym(\perm{132}{213}) & 8 & 1, 4, 28, 256, 2704, 31192, \ensuremath{\cdots} & \ensuremath{new} \\
\hline

